Obfuscated Access and Search Patterns in Searchable Encryption

Searchable Symmetric Encryption (SSE) allows a data owner to securely outsource its encrypted data to a cloud server while maintaining the ability to search over it and retrieve matched documents. Most existing SSE schemes leak which documents are accessed per query, i.e., the so-called access pattern, and thus are vulnerable to attacks that can recover the database or the queried keywords. Current techniques that fully hide access patterns, such as ORAM or PIR, suffer from heavy communication or computational costs, and are not designed with search capabilities in mind. Recently, Chen et al. (INFOCOM'18) proposed an obfuscation framework for SSE that protects the access pattern in a differentially private way with a reasonable utility cost. However, this scheme leaks the so-called search pattern, i.e., how many times a certain query is performed. This leakage makes the proposal vulnerable to certain database and query recovery attacks. In this paper, we propose OSSE (Obfuscated SSE), an SSE scheme that obfuscates the access pattern independently for each query performed. This in turn hides the search pattern and makes our scheme resistant against attacks that rely on this leakage. Under certain reasonable assumptions, our scheme has smaller communication overhead than ORAM-based SSE. Furthermore, our scheme works in a single communication round and requires very small constant client-side storage. Our empirical evaluation shows that OSSE is highly effective at protecting against different query recovery attacks while keeping a reasonable utility level. Our protocol provides significantly more protection than the proposal by Chen et al.~against some state-of-the-art attacks, which demonstrates the importance of hiding search patterns in designing effective privacy-preserving SSE schemes.

==> sections/conclusions.tex <==
\section{Conclusions}
Searchable symmetric encryption allows a data owner to outsource its data to a cloud server while maintaining the ability and therefore to search over it. Most existing SSE schemes leak access patterns, and therefore are vulnerable to attacks like the IKK attack. Oblivious RAM can be used to construct SSE scheme that fully hides access patterns. However such schemes suffer from heavy communication overhead making them impractical. \citeauthor{chen2018differentially} proposed an obfuscation framework to protect existing SSE schemes against access-pattern leakage. The framework can produce differentially private access patterns per keyword. However, it cannot hide whether the same keyword is being searched multiple times or, in other words, the search patterns. 

In this work, we proposed a stronger security definition for differentially private searchable symmetric encryption scheme and presented a real construction, $\DPSSE$, fulfilling it. On the one hand, $\DPSSE$ is adaptively semantically secure and provides differential privacy for both keywords and documents implying search-pattern hiding and access-pattern hiding. On the other hand, $\DPSSE$ has communication overhead as small as $O(\log\log n)$ and computation complexity of $O(n \cdot \log\log n)$ while searching for relatively frequent keywords. When assuming queries follow Zipfian distribution, the amortized communication overhead would be $O(\log n \log\log n)$. By replicating the IKK attack, we showed that our proposed scheme could actually hide access patterns and make it difficult for the server to extract useful information from differentially private access-pattern leakage. By performing KMeans clustering, we were able to show that inferring search patterns from differentially private access pattern leakage is difficult, namely search patterns are hidden. 

